Learning adaptive planning representations with natural language guidance

Effective planning in the real world requires not only world knowledge, but the ability to leverage that knowledge to build the right representation of the task at hand. Decades of hierarchical planning techniques have used domain-specific temporal action abstractions to support efficient and accurate planning, almost always relying on human priors and domain knowledge to decompose hard tasks into smaller subproblems appropriate for a goal or set of goals. This paper describes Ada (Action Domain Acquisition), a framework for automatically constructing task-specific planning representations using task-general background knowledge from language models (LMs). Starting with a general-purpose hierarchical planner and a low-level goal-conditioned policy, Ada interactively learns a library of planner-compatible high-level action abstractions and low-level controllers adapted to a particular domain of planning tasks. On two language-guided interactive planning benchmarks (Mini Minecraft and ALFRED Household Tasks), Ada strongly outperforms other approaches that use LMs for sequential decision-making, offering more accurate plans and better generalization to complex tasks.

==> backup/1-intro-bak-3.tex <==
\begin{abstract}
% First sentence -- too hard to understand, too many Ls, and too syntactically complex.
Long-horizon planning is dauntingly hard -- it requires modeling relevant aspects of the environment and searching over large, complex action spaces. \textit{Hierarchical planning} approaches make complex problems more tractable using temporal \textit{action abstractions}, decomposing hard tasks into smaller abstract subproblems that can be solved modularly. However, actually learning useful action abstractions has long posed significant challenges without human expert knowledge. Here, we introduce a system that leverages background information in language to learn a \textit{library of symbolic action abstractions and accompanying low-level policies} that can be composed to solve increasingly complex tasks. Our approach queries large language models (LLMs) as a prior for proposing useful symbolic action definitions, but integrates these proposals into a formal hierarchical planning system to ground and verify proposed actions. On two language-guided interactive planning domains (\textit{Mini Minecraft} and the \textit{ALFRED Household Tasks} benchmark), our approach far outperforms other baseline approaches that use LLMs in planning, enabling far more accurate planning and enable better generalization to more complex tasks.
% Jiayuan abstract 
% This paper proposes a novel approach to facilitate long-horizon planning by leveraging Large Language Models (LLMs) to guide the learning of hierarchical action abstraction. We employ LLMs as an Internet-scale knowledge base to extract planning-compatible and grounded action abstractions that are inherently enriched with common-sense knowledge about task decomposition. In particular, we integrate LLMs with a bi-level task and motion planning framework to generate a library of high-level actions represented using the Planning Domain Description Language (PDDL), allowing the actions to be human-interpretable, grounded, and sequentially chained to make long-horizon plans. We also introduce a hierarchical prompting strategy for generating a diverse set of high-level action descriptions. We show that the learned library of action abstractions can be adeptly recombined to resolve tasks of increased complexity.
% \lcw{This looks great! Will take another pass on this today}


% How do we do long horizon planning? We want natural action abstractions.
% LLMs provide a novel way to draw on world knowledge to propose these decompositions in reusable parts.
% But: how should they be represented and used? We argue that they should follow hierarchical TAMP -- we should learn operators and then learn policies coupled to them.
% This allows: efficient high level planning; contextual, grounded low-level planning.
% We introduce a prompting regime for  an initial set of diverse operators and then refine, verify, and ground these by using hierarchical planning.
% We find this works on two domains, both in a continual learning paradigm where we learn operators online.
% This outperforms all the other natural splits: decomposition radically cuts down on search time, improves over asking the LLM to plan, and is better than other modular librariers like imperative policies.
%------
% LCW: emphasize \textit{why} we have decomposed it this way. Language is the right way to overcome the robotics challenge of hand-designing world knowledge.
% And *specifically*, to learn libraries of composable subskills.
% But hierarchical planners are the right way to use and ground that knowledge in ways that are accurate, efficient, obey world state, and generalize to longer horizon plans.
% We find that this learns an effective, grounded, verified library that generalizes to hard tasks.
% And that it outperforms every other version of this -- using LLMs to directly predict any other part.
\end{abstract}

==> backup/1-intro-bak1.tex <==
\section{Introduction}


\lcw{work on this introduction and make some figures.
Dream of solving long horizon tasks with compositional skills.
For humans, language plays a role in this. Huge amount of prior knowledge.
Prior knowledge about how to \textit{decompose problems into subproblems}. Very general.
Prior knowledge about \textit{what} a given task is.
But actually using skills learned from language to solve tasks means \textit{grounding} them. Often grounding is domain-specific. Doing something in a video game requires mastering specific controllers; doing something in a particular environment is not the same as at home. Also contextual, dependent on particulars around you.
}

\jiayuan{Okay I have another idea about the intro. New story: LLMs contain a large amount of world knowledge, that can potentially benefit decision-making of interactive agents. However, there are a few challenges if we would like to use them as world models: they are not grounded and even incorrect due to its noisy nature, direct search in the language space can be inefficient. Therefore, we propose our new model. For the title, how about Hierarchical Planning with World Models from Word Models; or Grounded Planning with Hierarchical World Models from Word Models; or Hierarchical Planning Abstractions from Language Models?}

\lcw{Haha, yes. I like that intro and jotted a similar version of it down in the codex and skills doc this morning during lab meeting as well. Though idk about the phrase world models here -- it feels like we are learning something closer to grounded action abstractions. How do we solve complex problems? This has been the dream of much of planning. Decompose problems, and learn reusable skills, to boot — you enter a kitchen for the first time, and you ground all these skills, and then you produce a more complex dish; you play a game, and then you successively beat higher levels. This is the kind of thing you might think language models might be really good at. It knows about the world, it knows about words and can use that to guide decomposition, it knows about general code, it can even be prompted. But there are some things that it might seem undesirable for us to learn from a language model at all . Adapting that general knowledge to a specific setting; and solving planning itself. The problem requires knowing about high-level dependencies between actions that are what planning is all about; and low-level search that might just be very context specific and requires low-level feedback, and its inefficient to route all of that through language. In this project, we: Develop a method to extract skills. We extract them as PDDL operators. Allows us to draw on high level world knowledge in language. But we ground these out by both verifying them and learning coupled motion policies. This allows us to leverage planners. It also allows us to adaptively learn grounding over these high level actions into lower level ones.  We verify this on two domains. It’s much better than asking the LLM to do these directly, including just}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=1.0\textwidth]{figures/splash.pdf}
\end{center}
\vspace{-1em}
\caption{\lcw{Draft figure showing layout - temporary. Trying something different soon.}}
\label{fig:splash}
\end{figure}

The ability to make and execute long-horizon plans presents a grand challenge for the AI community. Various declarative programming and learning-based approaches, such as hierarchical task networks, hierarchical reinforcement learning, and hierarchical planning, have been proposed to tackle this issue. A profound concept underlying most of these methods is the development of {\it temporal (or action) abstractions}. Consider the simplest bi-level approach: the agent possesses a library of high-level actions that function at a broad temporal granularity (\eg, heat water, pour water, \etc, which are sometimes referred to as {\it task-level} actions). Additionally, there's a set of low-level actions that can be directly executed in the environment (\eg, move the robot arm, often termed as {\it motion-level} actions). When presented with a new task, which might be described in human language instructions (\eg, make some tea), the agent initially creates a plan at the task level, and then refines this task plan into low-level action plans.

An extensive body of research has been exploring how to learn and plan with such bi-level action spaces. In particular, in robotic task and motion planning, these abstractions are typically defined by domain experts using a symbolic programming language. In the context of hierarchical reinforcement learning, these abstractions are typically learned through hierarchical policy models or auxiliary losses. Despite being greatly useful, automatic learning of ``good'' action abstractions is inherently challenging without any human prior knowledge. This is because the hypothesis space of possible high-level actions grows exponentially with the time horizon. There are numerous criteria for these abstractions: high-level actions should be composable to produce long-horizon plans, planning with them should be time-efficient, and their corresponding sub-goals should be reliably achievable based on the motion-level action space, among other factors.

In this paper, we introduce an approach that leverages pretrained large language models (LLMs) as an Internet-scale knowledge base, to guide the learning of a planning-compatible and grounded action abstraction for interactive domains. We frame our problem in the style of reinforcement learning. Our agent can interact with an environment and has a dataset of tasks. Every task is described using a natural language instruction. The agent can explore the environment and attempt different tasks and will receive reward feedback upon successfully completing a task. Additionally, the agent has access to a library of predicates, which can describe the state of the environment, such as object categories and spatial relationships between objects.

The learning objective, therefore, is to build a library of planning-compatible and grounded high-level actions. Specifically, these high-level actions will be represented using the Planning Domain Description Language (PDDL): each action has an associated precondition (a classifier examining the current state to determine if the action is executable) and an effect (a description of the action's outcome). This situation calculus-style formalization ensures that high-level actions can be sequentially chained together based on their preconditions and effects, facilitating long-horizon planning. Moreover, these high-level actions are grounded: for each of them, we train a local policy that achieves the action's effect by predicting a sequence of low-level actions. By leveraging the library of high-level action descriptions in PDDL and their corresponding low-level policies, we can efficiently and effectively make and execute long-horizon plans for new tasks, and in unprecedented scenarios.

Our key idea is to leverage LLMs as a prior distribution for potentially useful high-level actions. In particular, we design a hierarchical prompting technique capable of producing a comprehensive set of potential high-level action descriptions based solely on the dataset of task descriptions. We then attempt to plan with and execute various high-level action proposals, selecting those that lead to the successful completion of tasks. Once learned, this library of actions can be directly applied to achieve new goals in the same environment, possibly requiring a larger planning horizon than those training tasks. Furthermore, since the high-level abstractions are represented in PDDL programs, both the action abstraction and the resulting plans are human-interpretable. This provides room for human intervention and diagnostic evaluation.

The contributions of the paper are the following. First, we proposed a novel approach that leverages Large Language Models (LLMs) to guide the learning of hierarchical action abstraction in interactive domains. Second, we introduce a hierarchical prompting strategy capable of generating a wide array of human-interpretable high-level action descriptions from task descriptions. We further integrated the prompting framework with a bi-level task and motion planning framework to select useful and correct action abstractions. Finally, we demonstrate that the learned action abstractions can be recombined to solve more complicated tasks.



==> backup/1-intro-bak2.tex <==
\section{Introduction}
The ability to make and execute long-horizon plans presents a grand challenge for the AI community. Various declarative programming and learning-based approaches, such as hierarchical task networks, hierarchical reinforcement learning, and hierarchical planning, have been proposed to tackle this issue. A profound concept underlying most of these methods is the development of {\it temporal (or action) abstractions}, which essentially decompose a complex task into smaller pieces that can be solved or learned to solve hierarchically.

% Consider the simplest bi-level approach: the agent possesses a library of high-level actions that function at a broad temporal granularity (\eg, heat water, pour water, \etc, which are sometimes referred to as {\it task-level} actions). Additionally, there's a set of low-level actions that can be directly executed in the environment (\eg, move the robot arm, often termed as {\it motion-level} actions). When presented with a new task, which might be described in human language instructions (\eg, make some tea), the agent initially creates a plan at the task level, and then refines this task plan into low-level action plans.

An extensive body of research has been exploring how to learn and plan with such abstract action spaces. In particular, in robotic task and motion planning, these abstractions are typically defined by domain experts using a symbolic programming language. In the context of hierarchical reinforcement learning, these abstractions are typically learned through hierarchical policy models or auxiliary losses. Despite being greatly useful, automatic learning of ``good'' action abstractions is inherently challenging without any human prior knowledge. This is because the hypothesis space of possible high-level actions grows exponentially with the time horizon. There are numerous criteria for these abstractions: high-level actions should be composable to produce long-horizon plans, planning with them should be time-efficient, and their corresponding sub-goals should be reliably achievable based on the motion-level action space, among other factors. \jiayuan{Two parts: traditional algorithms ..., LLMs ..., and they both have their own limitations.}

In this paper, we introduce an approach that leverages pretrained large language models (LLMs) as an Internet-scale knowledge base, to guide the learning of a planning-compatible and grounded action abstraction for interactive domains. Pretrained LLMs encapsulate a large amount of common-sense knowledge about everyday task decomposition. However, they are not directly grounded in the target domain, and even sometimes incorrect due to their noisy nature. Therefore, our goal in this paper is to build a system that can automatically extract action abstractions from LLMs and explorations in the environment, and leverage them to solve compositionally more complex tasks faster.

\input{fig-text/teaser}

To this end, we frame our problem in the style of reinforcement learning. Our agent can interact with an environment and has a dataset of tasks. Every task is described using a natural language instruction. The agent can explore the environment and attempt different tasks and will receive reward feedback upon successfully completing a task. Additionally, the agent has access to a library of predicates, which can describe the state of the environment, such as object categories and spatial relationships between objects.
The learning objective, therefore, is to build a library of planning-compatible and grounded high-level actions. Specifically, these high-level actions will be represented using the Planning Domain Description Language (PDDL): each action has an associated precondition (a classifier examining the current state to determine if the action is executable) and an effect (a description of the action's outcome). This situation calculus-style formalization ensures that high-level actions can be sequentially chained together based on their preconditions and effects, facilitating long-horizon planning. Moreover, these high-level actions are grounded: for each of them, we train a local policy that achieves the action's effect by predicting a sequence of low-level actions. By leveraging the library of high-level action descriptions in PDDL and their corresponding low-level policies, we can efficiently and effectively make and execute long-horizon plans for new tasks, and in unprecedented scenarios.

Our key idea is to leverage LLMs as a prior distribution for potentially useful high-level actions. In particular, we design a hierarchical prompting technique capable of producing a comprehensive set of potential high-level action descriptions based solely on the dataset of task descriptions. We then attempt to plan with and execute various high-level action proposals, selecting those that lead to the successful completion of tasks. Once learned, this library of actions can be directly applied to achieve new goals in the same environment, possibly requiring a larger planning horizon than those training tasks. Furthermore, since the high-level abstractions are represented in PDDL programs, both the action abstraction and the resulting plans are human-interpretable. This provides room for human intervention and diagnostic evaluation.

The contributions of the paper are the following. First, we proposed a novel approach that leverages Large Language Models (LLMs) to guide the learning of hierarchical action abstraction in interactive domains. Second, we introduce a hierarchical prompting strategy capable of generating a wide array of human-interpretable high-level action descriptions from task descriptions. We further integrated the prompting framework with a bi-level task and motion planning framework to select useful and correct action abstractions. Finally, we demonstrate that the learned action abstractions can be recombined to solve more complicated tasks.



==> backup/abstract-icml-original.tex <==
Long-horizon planning is dauntingly hard -- it requires modeling relevant aspects of the environment and searching over large, complex action spaces. \textit{Hierarchical planning} approaches make complex problems more tractable using temporal \textit{action abstractions}, decomposing hard tasks into smaller abstract subproblems that can be solved modularly. However, actually learning useful action abstractions has long posed significant challenges without human expert knowledge. Here, we introduce a system that leverages background information in language to learn a \textit{library of symbolic action abstractions and accompanying low-level policies} that can be composed to solve increasingly complex tasks. Our approach queries large language models (LLMs) as a prior for proposing useful symbolic action definitions, but integrates these proposals into a formal hierarchical planning system to ground and verify proposed actions. On two language-guided interactive planning domains (\textit{Mini Minecraft} and the \textit{ALFRED Household Tasks} benchmark), our approach far outperforms other baseline approaches that use LLMs in planning, enabling far more accurate planning and enable better generalization to more complex tasks.

==> backup/intro-icml-original.tex <==
People make plans over incredibly long and complex timescales, which govern how we act in granular
ways. To satisfy our vague hunger in the morning, we might ultimately execute tens of fine-grained
actions to open a fridge, locate and crack an egg, flip a pan, and then plate and fork up an omelet; to
satisfy our boss, we might plan a routine over days or even weeks that simply begins with navigating
a car to work. The general problem of forming and executing long, extended, and complex plans is
one of the unifying challenges of AI. It requires knowing what is relevant to represent in the world,
representing goals and utilities, and searching over actions in complex and uncertain environments.
While decades of research have developed many approaches for solving more restricted and shorter
term planning problems, general and extended long-horizon planning remains a core, outstanding
challenge for essentially all AI paradigms, including classical symbolic planning (Erol et al., 1994),
reinforcement learning (Sutton et al., 1999), and modern generative AI (Wang et al., 2023).
How do people solve this computational problem? One powerful idea developed across many AI
literatures is that of hierarchical planning using temporal action abstractions — that is, decomposing
complex tasks into smaller pieces that can be solved by progressively refining abstract subproblems
into sequences of lower-level actions. An extensive body of research has explored how to learn
and plan using these hierarchical action spaces, including a large body of robotic task-and-motion
planning (TAMP) systems (Garrett et al., 2021) and hierarchical RL frameworks (Sutton et al., 1999).
While the right abstractions can be immensely powerful for long-horizon planning and generalization
to new tasks, actually obtaining useful action abstractions poses one of the central bottlenecks in
general hierarchical planning. “Good” action abstractions must satisfy many different criteria: among
other factors, high-level actions should be composable to produce long-horizon plans, planning with
them should be time-efficient, and their corresponding sub-goals should be reliably achievable based
on the motion-level action space. Despite efforts to learn these abstractions automatically in both
classical planning (Nejati et al., 2006) and RL formulations (Dietterich, 2000), the problem of finding
useful action abstractions remains extremely challenging over longer time horizons without human
prior knowledge about the world and the problems a future agent might wish to solve.


In this paper, we frame the abstraction learning problem within a multitask-reinforcement-learning
objective. We consider settings in which an agent can interact with an environment and wishes to
solve a dataset of tasks of varying complexity. Each task is described using a high-level natural
language specification. The agent can explore the environment, attempting different tasks over time,
and will receive reward feedback upon successfully completing a task. Additionally, we assume
access to a set of symbolic predicates that describe general aspects of the environment state, such
as object categories and spatial relationships between objects. Our learning objective is to build a
library of planning-compatible and grounded actions. Specifically, we aim to learn actions with two
components: a high-level action abstraction represented as a symbolic planning operator (Fikes &
Nilsson, 1971) that specifies preconditions and action effects as sets of symbolic predicates; and
a low-level local policy that can achieve the action’s effects by predicting a sequence of low-level
actions. By leveraging the growing library of abstract actions, the agent ideally learns actions that can
be composed to efficiently make long-horizon plans for new tasks under new environment conditions.
Our core contribution is to show how we can use large language models (LLMs) to solve a key
part of the abstraction learning problem – as a powerful prior for proposing good symbolic operator
definitions on everyday planning domains. This allows our system to leverage the vast range of useful,
abstract world knowledge relevant to planning that is available in language, including commonsense
priors for decomposing tasks (e.g., that a cooking task might decompose into tasks for finding
ingredients, picking them up, and heating them) and for the abstract preconditions and effects of these
actions (e.g. that heating ingredients might be accomplished by putting them in a microwave, and
will result in the ingredients being hot). Equally importantly, however, our approach integrates LLMs
into a formal hierarchical planning framework, allowing us to leverage a powerful toolkit of efficient
planning methods to compose high-level actions, learn low-level policies, and verify learned actions.
Taken together, our system leverages language to learn a library of symbolic action abstractions and
accompanying local low-level policies that can be composed to solve increasingly complex tasks.
We evaluate our framework (Fig. 1) on two benchmarks, Mini Minecraft and ALFRED (Shridhar
et al., 2020). We compare our approach against three baselines that incorporate language models into
planning in other ways: to parse linguistic goals into formal specifications that are solved directly by
a planner (as in Liu et al. (2023)), to directly predict sequences of high-level subgoals (as in Ahn
et al. (2022)), and to predict libraries of actions defined in general imperative code (as in Wang et al.
(2023)). In both domains, we show that our approach learns action abstractions that allow it to solve
dramatically more tasks on each benchmark than these baselines, and that these abstractions compose
to permit much more efficient and accurate planning on more complex, unseen tasks.

==> fig-text/minecraft.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\textwidth]{figs/minecraft.pdf}
    \caption{(a) Visualization of our Mini Minecraft environment; the screenshot shows an intermediate step towards the goal ``{\it craft a bed.}'' (b) Visualization of an operator proposed by LLM and verified by our algorithm through planning and execution. (c) Visualization of the low-level crafting tools involved in the crafting of the bed. Resources dependencies such as {\it tree} and {\it iron ore vein} are omitted for brevity.}
    \label{fig:minecraft}
\end{figure}

==> fig-text/tab-minecraft.tex <==
\begin{table}[tp]
\centering
\small
\setlength{\tabcolsep}{8.4pt}
\begin{tabular}{llcccc}
\toprule
 & \textbf{LLM Predicts?} & \textbf{Library?} & \textbf{Mining} & \textbf{Crafting} & \textbf{Compositional} \\
\midrule
Motion Planning Only & Goal & \xmark & 31\% & 9\% & 9\% \\
% or 0%, 5% if we set max_expanded_nodes=1e3
Subgoal Prediction & Sub-goals & \xmark & 33\% & 31\% & 5\% \\
Voyager & Sub-policies & \cmark & 15\% & 42\% & 0\% \\
Ours & Goal+Operators & \cmark & 100\% & 100\% & 100\% \\
\bottomrule
\end{tabular}
\caption{Results on Mini Minecraft. Our algorithm successfully recovers all required operators in both mining and crafting tasks, and they enable generalization to more compositional tasks that require at most 26 high-level operators, without any additional learning.}
\label{tab:minecraft}
\end{table}
